Geometric analysis of generic 3R robots, and necessary and sufficient conditions for a class of orthogonal robots to have four IKS

The kinematic analysis of a generic 3R robot has been investigated with multiple approaches in the past. The algebraic approaches have established concrete results but are unfortunately limited to special classes or architectural simplifications. Geometric approaches on the other hand have extended the analysis to generic robots while also providing an intuitive understanding of their kinematic properties. We use the best of both approaches to present the kinematic analysis of a generic 3R robot, using the inverse kinematic model inherited from a method based on conformal geometric algebra. The paper discusses a generic framework to study the conditions for a 3R robot to have four inverse kinematic solutions (IKS) and allows to study the distribution of IKS as seen in workspace. The necessary and sufficient conditions for a class of orthogonal robots are presented using the proposed approach.

==> sections/3_classification.tex <==
\section{Classification of 3R robots based on number of IKS}
\label{sec:classification}

% \section{Conditions to have four IKS}
% As shown in the previous section, the position inverse kinematics of 3R robots is solved as the intersection of $\mv{C}_B$ and a circle obtained by rotating $\mv{C}_A$ about the second joint axis. This leads to a quartic polynomial in $\theta_2$ with coefficients as functions of DH parameters. It is still an open question to determine the necessary and sufficient conditions between the DH parameters to have 0, 2 or 4 real IK solutions due to the computational complexity of analyzing the quartic. However, it has been accomplished for orthogonal 3R robots~\cite{Phillip} but the complexity of the algebraic conditions does not give any intuition on the existence of a certain number of IKS. Therefore, we seek a geometric approach to do so and hence consider the problem as the intersection of a torus formed by rotating $\mv{C}_A$ about the second joint axis and the circle $\mv{C}_B$. 

% \subsection{Case $d_2 = d_3 = 0$}

==> temp_text.tex <==
\iffalse
Recalculating the Gr\"obner basis yields five polynomials of which the first two factor as follows:
\begin{align}
g_1 &=  g_{10} \, g_{11}\,g_{12}\, g_{13}\,g_{14} \mbox{ and } g_2 = y\,g_{10} \mbox{ with} \nonumber \\  g_{10} &= {r_{{B}}}^{4}+ \left( 2\,{R}^{2}-2\,{r}^{2}+2\,{z}^{2}-2\,{a_{{1}}}^{2
} \right) {r_{{B}}}^{2}+{a_{{1}}}^{4}-2\,{R}^{2}{a_{{1}}}^{2}+2\,{r}^{
2}{a_{{1}}}^{2} \nonumber  \\ 
& \hspace{0.5cm} +2\,{z}^{2}{a_{{1}}}^{2}+{R}^{4}-2\,{R}^{2}{r}^{2}-2\,{
R}^{2}{z}^{2}+{r}^{4}-2\,{r}^{2}{z}^{2}+{z}^{4} \nonumber \\  
g_{11} &=  (r_B - a_1)^2 - (R-r)^2 + z^2 \nonumber \\  
g_{12} &= (r_B - a_1)^2 - (R+r)^2 + z^2   \nonumber \\  
g_{13} &= (r_B + a_1)^2 - (R-r)^2 + z^2 \nonumber \\  
g_{14} &= (r_B + a_1)^2 - (R+r)^2 + z^2 
\end{align}
$g_2=0$ implies $y=0$ or $g_{10}=0$. Since we are interested in tangential extremes to cover all possible intersections, we only consider the intersections happening on the x-axis, i.e. $y=0$. Therefore to make $g_1=0$, one of the other factors $g_{1i}=0, i=\{1,2,3,4\}$ leading to eight solutions of $r_B$:
\begin{equation}
    r_B= \pm a_1 \pm \sqrt{(R \pm r)^2 - z^2}
\end{equation}
Substituting these values in~\eqref{eq:C_B} and eliminating $x$ from the obtained equation and $T_{A_{z=z_c}}$ leads to an equation in y. 
\fi
